OTAS: Unsupervised Boundary Detection for Object-Centric Temporal Action Segmentation

Temporal action segmentation is typically achieved by discovering the dramatic variances in global visual descriptors. In this paper, we explore the merits of local features by proposing the unsupervised framework of Object-centric Temporal Action Segmentation (OTAS). Broadly speaking, OTAS consists of self-supervised global and local feature extraction modules as well as a boundary selection module that fuses the features and detects salient boundaries for action segmentation. As a second contribution, we discuss the pros and cons of existing frame-level and boundary-level evaluation metrics. Through extensive experiments, we find OTAS is superior to the previous state-of-the-art method by $41\%$ on average in terms of our recommended F1 score. Surprisingly, OTAS even outperforms the ground-truth human annotations in the user study. Moreover, OTAS is efficient enough to allow real-time inference.

==> 06inplementation.tex <==
\section{Implementation Details}
\subsection{Global Perception Module}
\noindent\textbf{Architecture.} The spatial encoder is a ResNet50 model~\citep{he2016deep} with 2048 output classes. The temporal decoder is adapted from the Transformer~\citep{vaswani2017attention} with 2048 hidden dimensions and 8 heads. The decoder is constructed by stacking 6 up-sampling blocks. Each block contains an up-sampling function, a convolution layer, and a ReLU activation function. The kernel size is 7 for the first and last blocks and 3 for the rest. The interpolation sizes are 8, 16, 32, 64, 128, and 256, sequentially. The channels are 1024, 512, 256, 128, 64, and 3, respectively. \\

\noindent\textbf{Optimizer and schedule.} We use the standard Adam~\cite{kingma2014adam} optimizer with a learning rate of 1e-4 and a multi-step scheduler. We train the model for a total of 250000 steps with a batch size of 16.\\

\begin{comment}
{\footnotesize
architecture = \{
\par \qquad ``ResNet'' : \{
\par \qquad \qquad ``block'': Bottleneck,
\par \qquad \qquad``layers'': [3,4,6,3],
\par \qquad \qquad``num\_classes'': 2048,
\par \qquad \qquad``zero\_init\_residual'': False,
\par \qquad \qquad``groups'': 1,
\par \qquad \qquad``width\_per\_group'': 64,
\par \qquad \qquad``replace\_stride\_with\_dilation'': None,
\par \qquad \qquad``norm\_layer'' : BatchNorm2d
\par \qquad \},
\par \qquad ``PositionalEncoding : \{
\par \qquad \qquad ``d\_model'': 2048,
\par \qquad \qquad``max\_length'': 5,
\par \qquad \qquad``dropout'': 0.1,
\par \qquad \},
\par \qquad ``TransformerEncoderLayer : \{
\par \qquad \qquad ``d\_model'': 2048,
\par \qquad \qquad``nhead'': 8,
\par \qquad \qquad``dim\_feedforward'': 2048,
\par \qquad \qquad``dropout'': 0.1,
\par \qquad \qquad``activation'': relu,
\par \qquad \qquad``layer\_norm\_eps'': 1e-5,
\par \qquad \},
\par \qquad ``Decoder'' : \{
\par \qquad \qquad ``interpolate\_mode'': bilinear,
\par \qquad \qquad ``align\_corners'': False,
\par \qquad \qquad ``stride'': 1,
\par \qquad \qquad ``padding'': 3,
\par \qquad \qquad ``norm\_layer'': BatchNorm2d,
\par \qquad \qquad ``activitation'': relu,
\par \qquad \qquad ``blocks'':[
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 8,
\par \qquad \qquad \qquad  ``channels'': 1024,
\par \qquad \qquad \qquad  ``kernel\_size'': 7
\par \qquad \qquad \quad  \}, 
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 16,
\par \qquad \qquad \qquad  ``channels'': 512,
\par \qquad \qquad \qquad  ``kernel\_size'': 3
\par \qquad \qquad \quad  \},
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 32,
\par \qquad \qquad \qquad  ``channels'': 256,
\par \qquad \qquad \qquad  ``kernel\_size'': 3
\par \qquad \qquad \quad  \},
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 64,
\par \qquad \qquad \qquad  ``channels'': 128,
\par \qquad \qquad \qquad  ``kernel\_size'': 3
\par \qquad \qquad \quad  \},
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 128,
\par \qquad \qquad \qquad  ``channels'': 64,
\par \qquad \qquad \qquad  ``kernel\_size'': 3
\par \qquad \qquad \quad  \},
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 256,
\par \qquad \qquad \qquad  ``channels'': 3,
\par \qquad \qquad \qquad  ``kernel\_size'': 7
\par \qquad \qquad \quad  \}
\par \qquad \qquad ]
\par \qquad \}
\par \}

\vspace*{1\baselineskip}
\par learning\_rate=optim.lr\_scheduler.MultiStepLR(
\par \qquad milestones = [100000],
\par \qquad gamma = 0.1)

\vspace*{1\baselineskip}
\par optimizer=optim.Adam(
\par \qquad lr = 1e-4,
\par \qquad weight\_decay = 1e-4)
}

\end{comment}

\subsection{Human-Object Interaction Model}
\noindent\textbf{Architecture.} The architecture of the human-object interaction model is the same as the global perception model without the decoder.\\

\noindent\textbf{Human-object interaction masks.} We obtain the masks from an off-the-shelf object detection model implemented by the open source platform Detectron2~\citep{wu2019detectron2}. We select the Faster-RCNN-X101-FPN model pre-trained on the COCO train2017 dataset~\citep{lin2014microsoft} with a box average precision (box AP) of 43.0. For human-object interaction, we select masks that contain human body parts, \eg \textit{person}. 


\subsection{Object Relationship Model}
\noindent\textbf{Architecture.} The encoder is also a ResNet50 model~\citep{he2016deep}, and the decoder is the same as the frame prediction model. We adapt architecture from GATv2~\citep{brody2021attentive} for graph implementation in the bottleneck part. We use two 8-heads self-attention layers, with 32 input channels and 6 output channels for each head. We then add a fully-connected layer to project the output to 2048 dimension.\\

\noindent\textbf{Optimizer and schedule.} We use the standard Adam~\cite{kingma2014adam} optimizer with a learning rate of 5e-5 and a multi-step scheduler. We train the model for a total of 100000 steps with a batch size of 16.\\

\noindent\textbf{Object relationship look-up table.} For all the object classes in COCO dataset~\citep{lin2014microsoft}, we select 44 classes that appear most frequently in instructional videos. All 44 classes are depicted in Table~\ref{coco classes}. We then seek their relations through human annotations from the Visual Genome dataset~\citep{krishna2017visual}, which is designed for cognitive tasks. To be more specific, we first re-organize the object classes of the Visual Genome dataset to be in line with the 44 classes we selected from the COCO dataset. Some examples of the re-organization are shown in Table~\ref{genome classes}. 
Then, for each class, we list and count all possible connections of the objects through predicates provided by the Visual Genome dataset. Finally, we filter out object pairs that appear less than 30 times and build the object relation look-up table. A few illustrations of the look-up table are illustrated in Table~\ref{dictionary}. 

\begin{table}[ht]
\footnotesize
  \centering
  \setlength{\tabcolsep}{0.6mm}
  \begin{tabular}{@{}|c|c|c|c|c|c|c|@{}}
  \hline
toothbrush&scissors&vase&clock&book&refrigerator&sink\\
\hline
toaster&oven&microwave&cell&keyboard&remote&mouse\\
\hline
laptop&tv&table&plant&couch&chair&cake\\
\hline
donut&pizza&hotdog&carrot&broccoli&orange&sandwich\\
\hline
apple&banana&bowl&spoon&knife&fork&cup\\
\hline
glass&bottle&suitcase&handbag&backpack&bench&person\\
\hline
rack&cabinet&~&~&~&~&~\\
\hline
  \end{tabular}
  \vspace{0.4mm}
  \caption{\textbf{New object classes selected from the COCO dataset.}}
  \label{coco classes}
\end{table}

\begin{table}[t]
\footnotesize
  \centering
  \setlength{\tabcolsep}{0.7mm}
  \begin{tabular}{@{}|l|@{}}
  \hline
person\\
\hline
person, man, woman\\
\hline
table\\
\hline
table, coffee\_table, counter, countertop, desk\\
\hline
knife\\
\hline
knife, steak\_knife, butter\_knife, knife\_blade, bread\_knife, butcher\_knife\\
\hline
  \end{tabular}
  \vspace{0.4mm}
  \caption{\textbf{Illustrations of the re-organization for the Visual Genome dataset.}}
  \label{genome classes}
\end{table}

\begin{table}[ht]
\footnotesize
  \centering
  \setlength{\tabcolsep}{0.7mm}
  \begin{tabular}{@{}|l|@{}}
  \hline
toothbrush\\
\hline
cup, sink, person, rack, table\\
\hline
cake\\
\hline
table, bowl, person, cup, knife, fork\\
\hline
knife\\
\hline
table, fork, person, cake, pizza, apple, orange, banana, sandwich\\
\hline
  \end{tabular}
  \vspace{0.4mm}
  \caption{\textbf{Illustrations of the object relationship look-up table.}}
  \label{dictionary}
\end{table}

%\noindent\textbf{Graph construction.} The two conditions that specify a relation between two object classes are a) the two object classes are related according to the object relation dictionary; b) the distance between the two objects in the frame is within a threshold of 80 pixels. We then build a graph for each frame regarding the relations. 

\noindent\textbf{Object masks.} We obtain the object masks from the same off-the-shelf object detection model~\citep{wu2019detectron2} as the human-object interaction model. We select masks that are in the new object classes and have confidence scores that are larger than 0.7. 

\begin{comment}
    

{\footnotesize
architecture = \{
\par \qquad ``ResNet'' : \{
\par \qquad \qquad ``block'': Bottleneck,
\par \qquad \qquad``layers'': [3,4,6,3],
\par \qquad \qquad``num\_classes'': 1024,
\par \qquad \qquad``zero\_init\_residual'': False,
\par \qquad \qquad``groups'': 1,
\par \qquad \qquad``width\_per\_group'': 64,
\par \qquad \qquad``replace\_stride\_with\_dilation'': None,
\par \qquad \qquad``norm\_layer'' : BatchNorm2d
\par \qquad \},
\par \qquad ``GATv2Conv1'' : \{
\par \qquad \qquad ``in\_channels'': 2048,
\par \qquad \qquad``out\_channels'': 32,
\par \qquad \qquad``heads'': 8,
\par \qquad \qquad``concat'': True,
\par \qquad \qquad``bias'': False,
\par \qquad \qquad``share\_weights'': True,
\par \qquad \qquad``dropout'' : 0.5
\par \qquad \},
\par \qquad ``GATv2Conv2'' : \{
\par \qquad \qquad ``in\_channels'': 32,
\par \qquad \qquad``out\_channels'': 6,
\par \qquad \qquad``heads'': 8,
\par \qquad \qquad``concat'': True,
\par \qquad \qquad``bias'': False,
\par \qquad \qquad``share\_weights'': True,
\par \qquad \qquad``dropout'' : 0.5
\par \qquad \},
\par \qquad ``fc'' : \{
\par \qquad \qquad ``in\_channels'': 2112,
\par \qquad \qquad``out\_channels'': 2048
\par \qquad \},
\par \qquad ``Decoder'' : \{
\par \qquad \qquad ``interpolate\_mode'': bilinear,
\par \qquad \qquad ``align\_corners'': False,
\par \qquad \qquad ``stride'': 1,
\par \qquad \qquad ``padding'': 3,
\par \qquad \qquad ``norm\_layer'': BatchNorm2d,
\par \qquad \qquad ``activitation'': relu,
\par \qquad \qquad ``blocks'':[
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 8,
\par \qquad \qquad \qquad  ``channels'': 1024,
\par \qquad \qquad \qquad  ``kernel\_size'': 7
\par \qquad \qquad \quad  \}, 
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 16,
\par \qquad \qquad \qquad  ``channels'': 512,
\par \qquad \qquad \qquad  ``kernel\_size'': 3
\par \qquad \qquad \quad  \},
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 32,
\par \qquad \qquad \qquad  ``channels'': 256,
\par \qquad \qquad \qquad  ``kernel\_size'': 3
\par \qquad \qquad \quad  \},
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 64,
\par \qquad \qquad \qquad  ``channels'': 128,
\par \qquad \qquad \qquad  ``kernel\_size'': 3
\par \qquad \qquad \quad  \},
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 128,
\par \qquad \qquad \qquad  ``channels'': 64,
\par \qquad \qquad \qquad  ``kernel\_size'': 3
\par \qquad \qquad \quad  \},
\par \qquad \qquad \quad  \{ 
\par \qquad \qquad \qquad  ``interpolate\_size'': 256,
\par \qquad \qquad \qquad  ``channels'': 3,
\par \qquad \qquad \qquad  ``kernel\_size'': 7
\par \qquad \qquad \quad  \}
\par \qquad \qquad ]
\par \qquad \}
\par \}

\vspace*{1\baselineskip}
\par learning\_rate=optim.lr\_scheduler.MultiStepLR(
\par \qquad milestones = [40000],
\par \qquad gamma = 0.1)

\vspace*{1\baselineskip}
\par optimizer=optim.Adam(
\par \qquad lr = 5e-5,
\par \qquad weight\_decay = 1e-4)
}

\end{comment}



%\subsection{Boundary Selection Model}  
%We select local maximums of the temporal feature difference with an interval $\alpha$ and a threshold $\theta$ to serve as boundary candidates. For Breakfast~\citep{kuehne2014language}, we set $\alpha=15$, and $\theta=51$
%For each boundary in the global visual set, if it has more than one neighbor, then we build a boundary cluster containing the boundary along with its neighbors. Within each boundary cluster, we select the one with the highest score as the final output. 



==> 07evaluation.tex <==
\section{Evaluation Metrics}
\subsection{F1 Score}
For the computation of the F1 score, we follow the implementation of \citet{shou2021generic, wang2021coseg} and first calculate the distance between the $N$ detected boundaries and the $M$ ground truth boundaries. We pair each ground truth boundary with a detected boundary that has a minimal distance. Then, we set a fixed distance threshold to determine if the detected boundary is positive or not. The total number of positive detection is $P$. The Precision/Recall and F1 score can be computed as:

\begin{align}
    &\text{precision}=\frac{P}{N} \notag \\
    &\text{recall}=\frac{P}{M} \notag \\
    &F_1=2\frac{\text{precision} \cdot \text{recall}}{\text{precision}+\text{recall}} \notag
\end{align}
We compute the Precision/Recall and F1 score for each video and average across the whole dataset. 

As mentioned in the paper, previous works~\citep{shou2021generic, wang2021coseg} set the distance threshold to be 5\% of the length of the corresponding video instance, while we choose 2 seconds which is invariant of video lengths. We show some examples in Figure~\ref{f1} for the impact of the 2 different thresholds. It is clear that the small threshold is more suitable and general for the evaluation of various instructional videos. 

\begin{figure}[t]
\centering
\includegraphics[height=3.8cm]{fig-supple/f1.pdf}
\caption{\textbf{Illustrations of different thresholds for the boundary-level F1 score.} For evaluation of the boundary ``Start of spoon powder'', it is clear that a 2s deviation is not harmful. However, a 22.3s threshold (5\% of a 7 min 26s video) will cause the boundaries even in ``Background'' and ``Take plate'' to be falsely labeled positive.}
\label{f1}
\end{figure}

\subsection{Hungarian Matching}
To perform a fair evaluation with previous methods utilizing clustering algorithms~\citep{kukleva2019unsupervised, sarfraz2021temporally, de2021cluster,du2022fast}, we first applying clustering algorithm as in ~\citet{du2022fast} to transfer OTAS boundaries into clusters based on IDT features. Then, we follow ~\citep{Aakur_2019_CVPR, wang2021coseg} and perform the Hungarian matching ~\citep{kuhn1955hungarian} on a video level. 

Noting that for other clustering-based methods that are either only performing on same activities ~\citep{sener2018unsupervised,kukleva2019unsupervised,elhamifar2019unsupervised,li2021action,vidalmata2021joint,wang2021unsupervised,swetha2021unsupervised,wang2022sscap, elhamifar2020self} or extend to unknown activities but only provide global-level Hungarian matching results and do not provide code to reproduce~\citep{kumar2021unsupervised, ding2021temporal}, we can not conduct a fair comparison. 

\begin{comment}
\subsection{Intersection over Union~(IoU)}
After the Hungarian matching, we can obtain a one-on-one matching of the ground truth clusters and the detected segments. IoU is computed as the mean intersection over union between all the detected and ground truth segments. For each segment, we set the intersection time interval as $I$ and union time interval as $U$, and the IoU for a video with $N$ ground-truth clusters is computed as:

\begin{equation}
    \text{IoU}=\frac{1}{N} \sum_{n=1}^N \frac{I_n}{U_n} \notag
\end{equation}
We then average across the whole dataset. 

While we target boundary detection, which treats all segments as different events. Clustering-based methods merge all similar events together. As illustrated in Figure~\ref{iou}, the person in a video takes out the fruit in a bowl when cutting fruits and resumes the cutting behavior afterwards. Clustering-based methods would merge two cutting segments into one, while event boundary detection methods tend to recognize them as separate events. The same situation happens for backgrounds at the start and end of the videos. Since we aim for boundary evaluation, this will cause a huge decrease in the performance of IoU. However, we still implement the same evaluation to compare with clustering-based methods.   

 \begin{figure}[htb]
\centering
\includegraphics[height=2.1cm]{draft/iou.pdf}
\caption{For this video, ``Background'', ``Cut fruit'', ``Peel fruit'', and ``Put fruit to bowl'' are all repeat events, which are assigned with the same label in the dataset. However, the unsupervised boundary detection method sees them as separate events. Therefore, all future repeat segments are treated as false segmentation regardless of the boundary.}
\label{iou}
\end{figure}
\end{comment}

\subsection{Mean over Frames~(MoF)}
We calculate MoF after clustering and Hungarian Matching. MoF indicates the percentage of frames in the video instance that are correctly segmented~\citep{sener2018unsupervised, kukleva2019unsupervised}. For a video with $K$ frames, we count all the correct frames $C$ and compute the MoF as: 
\begin{equation}
    \text{MoF}=\frac{C}{K} \notag
\end{equation}
We average the video-wise MoF across the whole dataset. 


==> 08user.tex <==
\section{User Study}
\subsection{Implementation}
We first pick 20 videos from the Breakfast dataset~\citep{kuehne2014language} randomly and generate segmented videos from 5 different methods: one from ground truth, one from OTAS, one from ABD~\citep{du2022fast}, one from CTE~\citep{kukleva2019unsupervised}, and the last one from TW-FINCH~\citep{sarfraz2021temporally}. For each video, We shuffle and label 5 segmentation results with numbers 1-5. We invite 33 users to watch and rank the segmentation results with only the reference to the original videos. A part of the user study questionnaire is depicted in Figure~\ref{user study interface}. Since it is a temporal segmentation task, the average time of completion is 2.5 hours. We use $6-rank$ as the score for each method (i.e., rank No.1 has 5 points). A video-wise score distribution is shown in Figure~\ref{video-wise}. We show one of our segmentation results that gains the highest score in Figure~\ref{user}.

\subsection{Breakfast Ground Truth}
We provide more illustrations of the inconsistent ground truth segmentation of the Breakfast dataset~\citep{kuehne2014language} in Figure~\ref{user_GT}.  

\begin{figure}[t]
\centering
\includegraphics[height=4cm]{fig-supple/interface.pdf}
\caption{\textbf{User study questionnaire interface.} We provide only the options to choose from, excluding any reference to the granularity information.}
\label{user study interface}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[height=4cm]{fig-supple/GT.pdf}
\caption{\textbf{Inconsistency of the ground-truth.} For ``Sandwich'' activity, the action ``Cut bun'' can be further segment into ``Take bun'', ``Take knife'', and ``Actually cut the bun''; while the action ``Smear butter'' can be further segment into ``Take butter'', ``Take knife'', and ``Actually smear the butter''. However, the ground truth annotation provides inconsistent segmentation that sometimes produces larger segments and sometimes smaller segments. Even within a video, the segmentation is inconsistent.}
\label{user_GT}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[height=7cm]{fig-supple/user.pdf}
\caption{\textbf{More consistent granularity of the segmentation results produced by OTAS.} The video shown in the figure contains several smaller segments at the action level. The ground truth only segments ``Take butter'' out, and combine the others, which is confusing while watching. Furthermore, the ground truth does not separate ``Take ingredients'' and ``Serve on plate'' from the backgrounds. However, our segmentation result is neat and consistent, which is more in line with human consensus. }
\label{user}
\end{figure*}





==> 09qualitative.tex <==
\begin{figure*}[t]
\centering
\includegraphics[height=8cm]{fig-supple/breakfast.pdf}
\caption{\textbf{Qualitative comparison with ground truth (GT) of the Breakfast dataset.} The results predicted by OTAS are largely in line with the ground truth.}
\label{breakfast}
\end{figure*}

\section{Qualitative Result}
For a better illustration of boundary evaluation, we assign all different ground truth segments distinct colors within a video regardless of labels. 
\subsection{Breakfast}
We provide more qualitative comparisons with the ground truth of our methods on the Breakfast dataset~\citep{kuehne2014language} in Figure~\ref{breakfast}. 

\subsection{50Salads}
The qualitative comparison of our methods on both eval-level and mid-level 50salads~\citep{stein2013combining} is illustrated in Figure~\ref{50salads}. For eval-level, we compare with baselines ABD~\citep{du2022fast}, CTE~\citep{kukleva2019unsupervised}, TW-FINCH~\citep{sarfraz2021temporally}, Coseg~\citep{wang2021coseg} and groundtruth. For mid-level, we only compare with  ABD~\citep{du2022fast}, CTE~\citep{kukleva2019unsupervised}, TW-FINCH~\citep{sarfraz2021temporally}, and ground truth, since Coseg~\citep{wang2021coseg} does not provide mid-level results. 

\subsection{INRIA}
The INRIA dataset~\citep{alayrac2016unsupervised} is collected from YouTube and segmented with the aid of English transcripts obtained from YouTube’s automatic speech recognition (ASR) system. For all tasks, the ordered sequence of ground truth steps is made by
an agreement of 2-3 annotators who have watched the input videos and verified the steps on instruction video websites. Therefore, the rest of the video where no step is assigned is considered background. The percentage of average background frames is 73\% of all frames. The background frames are various and complicated, as shown in Figure~\ref{INRIA}.  Since we rely on feature differences for boundary detection, the variation in backgrounds influences the result largely. Moreover, we do not have access to prior knowledge of cluster numbers. Therefore, the result of INRIA is very likely to be over-segmented. 


==> 10ablation.tex <==
\section{Ablation Study}
\subsection{Comparison of Different $\alpha$}
We utilize a hyper-parameter $\alpha$ to control the number of boundaries. The comparison of different $\alpha$ is shown in Tab.~\ref{Ablation alpha}. 
Generally, lower $\alpha$ leads to higher recall, but also redundancy, which causes precision to drop. Higher $\alpha$ generates fewer boundaries, resulting in higher precision and MoF but low recall. We select $\alpha=15$ that best balances the trade-off. 

\begin{table}[htbp]
\footnotesize
  \centering
  \setlength{\tabcolsep}{0.85mm}
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    ~& F1(\textit{small}) & Recall(small)&Precision(small)&MoF \\
    \midrule
    $\alpha=8$&42.43&\textbf{71.96}&30.08&65.22\\
    $\alpha=25$&42.77&48.31&\textbf{38.37}&67.57\\
    $\alpha=15$&\textbf{44.49}&53.90&37.87&\textbf{67.90}\\
    \bottomrule
  \end{tabular}
  \vspace{0.8mm}
  \caption{\textbf{Comparison of different $\alpha$s.} There is a trade-off between better precision and better recall.}
  \label{Ablation alpha}
\end{table}


\subsection{Global Perception Module Architectures}
We also conduct an ablation study on different model architectures for the global perception module. Specifically, we leverage features from pre-computed IDT, a pre-trained ResNet-50 model and ResNet with a 2-layer LSTM model that respectively replaces the Transformer layer for comparison. The results demonstrated in Table~\ref{Ablation structure} indicate that the Transformer-based model generates finer features for action segmentation than the other models. 

\begin{table}[ht]
\footnotesize
  \centering
  \setlength{\tabcolsep}{0.85mm}
  \begin{tabular}{@{}lcc@{}}
    \toprule
    ~& F1(\textit{small}) & MoF \\
    \midrule
    IDT&27.49&63.50\\
    Pretrained-ResNet&35.28&65.00\\
    LSTM&36.00&65.50\\
    Transformer&\textbf{37.46}&\textbf{65.99}\\
    \bottomrule
  \end{tabular}
  \vspace{0.8mm}
  \caption{\textbf{Ablation of different architectures for the global perception module (OTAS excluding the local attention module) on Breakfast.} Transformer-based approach achieves the best performance of F1 score and IoU.}
  \label{Ablation structure}
\end{table}

\begin{comment}
\begin{table}[ht]
\footnotesize
  \centering
  \setlength{\tabcolsep}{0.85mm}
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    ~ &\multicolumn{3}{c}{
    \textit{small threshold}}\\
    ~& F1 & Rec. & Prec.&MoF & IoU\\
    \midrule
    Interaction features&31.65&34.30&29.38&54.24&44.80\\
    Relationship features&38.67&42.63&35.39&56.01&49.42\\
    \bottomrule
  \end{tabular}
  \caption{Ablation study of different model architectures for boundary detection on Breakfast. The interaction features refer to the features generated from the pretrained ResNet50~\citep{he2016deep} with the same input as the human-object interaction model. So are relationship features with the object relationship model. }
  \label{model}
\end{table}
\end{comment}

\clearpage
\begin{figure*}[t]
\centering
\includegraphics[height=9cm]{fig-supple/50s.pdf}
\caption{\textbf{Qualitative comparison of the 50Salads dataset.} Note that the original illustration of Coseg is not aligned with the actual timestamp. However, since they do not provide code to reproduce, we roughly resize their illustration for comparison. }
\label{50salads}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[height=6.6cm]{fig-supple/inria.pdf}
\caption{\textbf{Illustration of the various background frames of INRIA.} It contains frames when the person shows preparation, stops to introduce upcoming steps, illustrates precautions, etc. It also contains shot changes and video editing.}
\label{INRIA}
\end{figure*}

\clearpage
\begin{figure*}[t]
\centering
\includegraphics[width=21cm, angle=270]{fig-supple/bar.pdf}
\vspace{2.8mm}
\caption{\textbf{Video-wise user study score.}}
\label{video-wise}
\end{figure*}
